AntEval: Evaluation of Social Interaction Competencies in LLM-Driven Agents

Large Language Models (LLMs) have demonstrated their ability to replicate human behaviors across a wide range of scenarios. However, their capability in handling complex, multi-character social interactions has yet to be fully explored, primarily due to the absence of robust, quantitative evaluation methods. This gap has slowed the development of agents proficient in more nuanced interactions beyond simple exchanges, for example, small talk. To address this challenge, we introduce the Multi-Agent Interaction Evaluation Framework (AntEval), encompassing a novel interaction framework and evaluation methods. The interaction framework aims to foster an complex interaction environment that bolsters information exchange and intention expression within social interactions. Furthermore, we introduce evaluation methods, including two metrics: Information Exchanging Precision (IEP) and Interaction Expressiveness Gap (IEG), designed for the quantitative and objective assessment of agents' interaction competencies. Our findings highlight the utility of these evaluative methods and show significant potential for improving LLMs' ability to construct agents that interact in a more natural manner with human-like intricacy.

==> bak.tex <==

% \begin{table}[]
% 	\begin{center}
% 	\resizebox{0.7\columnwidth}{!}
%       {
%         \begin{tabular}{|l|c|}
%         \hline
%         \multicolumn{1}{|c|}{Evaluation Model} & Mean Precision \\ \hline \hline 
%         LLaMA-7b                               & 0.36           \\ \hline
%         LLaMA-2-7b                             & 1.60           \\ \hline
%         LLaMA-2-13b                            & 3.83           \\ \hline
%         LLaMA-2-70b                            & 9.64           \\ \hline
%         Mistra-7B                              & 3.09           \\ \hline
%         Mixtral-8x7B                           & 8.68           \\ \hline
%         GPT-3.5                                & 55.93          \\ \hline
%         GPT-4                                  & 60.40          \\ \hline
%         \end{tabular}
%       }
%      \end{center}
%     \caption{Comparison for the mean precision of key point prediction in AntEval. }
%     \label{table::tab_mul_llm_avg_prec}
% \end{table}





% Moreover, as in Tab~\ref{table::tab_var}, we present the variance for calculate the mathching precision of key points. All the combinations of interaction model and summarization models show similar variances. These show the fluctuation in predictions and summarizations. Besides, though there are some fluctuations, all the fluctuations are relatiely stable and the variance are about $5$. These indicates that our evalutaion method is effective and relatively robustness. 

% \begin{table}[]
% 	\begin{center}
% 	\resizebox{0.9\columnwidth}{!}
%       {
%         \begin{tabular}{|l|ccc|}
%         \hline
%         \multicolumn{1}{|c|}{\multirow{2}{*}{Summarization Model}} & \multicolumn{3}{c|}{Evaluation Model}                                                \\ \cline{2-4} 
%         \multicolumn{1}{|c|}{}                                     & \multicolumn{1}{c|}{GPT-3.5} & \multicolumn{1}{c|}{GPT-4} & LLaMA \\ \hline \hline 
%         GPT-3.5                                                     & \multicolumn{1}{c|}{5.28}  & \multicolumn{1}{c|}{5.42}     &                            \\ \hline
%         GPT-4                                                       & \multicolumn{1}{c|}{10.55}       & \multicolumn{1}{c|}{4.44}     &                            \\ \hline
%         LLaMA                                                      & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{}     &                            \\ \hline
%         \end{tabular}
%         }
%         \end{center}
%     \caption{comparison for the variances of different models in our evaluation. }
%     \label{table::tab_var}
% \end{table}

% \begin{table*}[]
% 	\begin{center}
% 	\resizebox{2\columnwidth}{!}
%       {
%         \begin{tabular}{|l|ccccc|ccccc|}
%         \hline
%         \multicolumn{1}{|c|}{\multirow{2}{*}{Model}} & \multicolumn{5}{c|}{Character Prediction}                                                                                                 & \multicolumn{5}{c|}{Intention Prediction}                                                                                                 \\ \cline{2-11} 
%         \multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{$f_{0 \rightarrow r} (\uparrow)$} & \multicolumn{1}{c|}{$f_{v \rightarrow r} (\uparrow)$} & \multicolumn{1}{c|}{$f_{0 \rightarrow v} (\uparrow)$} & \multicolumn{1}{c|}{$f_{r \rightarrow v} (\uparrow)$} & $G (\downarrow)$     & \multicolumn{1}{c|}{$f_{0 \rightarrow r} (\uparrow)$} & \multicolumn{1}{c|}{$f_{v \rightarrow r} (\uparrow)$} & \multicolumn{1}{c|}{$f_{0 \rightarrow v} (\uparrow)$} & \multicolumn{1}{c|}{$f_{r \rightarrow v} (\uparrow)$} & $G (\downarrow)$   \\ \hline \hline 
%         GPT-3.5                                      & \multicolumn{1}{c|}{26.48}          & \multicolumn{1}{c|}{23.02}     & \multicolumn{1}{c|}{37.46}          & \multicolumn{1}{c|}{52.48}     & 24.48 & \multicolumn{1}{c|}{8.32}          & \multicolumn{1}{c|}{2.19}      & \multicolumn{1}{c|}{11.14}          & \multicolumn{1}{c|}{9.12}      & 36.34 \\ \hline
%         GPT-3.5 (long-context)                       & \multicolumn{1}{c|}{29.89}          & \multicolumn{1}{c|}{37.01}     & \multicolumn{1}{c|}{86.98}          & \multicolumn{1}{c|}{93.59}     & 0.39 & \multicolumn{1}{c|}{12.22}          & \multicolumn{1}{c|}{19.95}     & \multicolumn{1}{c|}{22.49}          & \multicolumn{1}{c|}{34.71}     & 8.21 \\ \hline
%         \end{tabular}
%      }
%      \end{center}
%     \caption{comparison for the gap of different models trained from real and generated interactions. GPT-3.5-lc indicates long-context version relased recently. $F_c$ indicates character F score, $F_i$ indicates interaction F score, $G_c$ indicates character prediction gap, and $G_i$ indicates interaction prediction gap. }
%     \label{table::tab_gap}
% \end{table*}




% \begin{table*}[]
% 	\begin{center}
% 	\resizebox{1.1\columnwidth}{!}
%       {
%         \begin{tabular}{|l|cc|cc|}
%         \hline
%         \multicolumn{1}{|c|}{\multirow{2}{*}{Model}}         & \multicolumn{2}{c|}{Character Prediction}       & \multicolumn{2}{c|}{Intention Prediction}       \\ \cline{2-5} 
%         \multicolumn{1}{|c|}{}             & \multicolumn{1}{c|}{$f_v (\uparrow)$} & $G (\downarrow)$ & \multicolumn{1}{c|}{$f_v (\uparrow)$} & $G (\downarrow)$ \\ \hline \hline 
%         LLaMA-2-7b                           & \multicolumn{1}{c|}{13.51}   &  49.25                     & \multicolumn{1}{c|}{0.90}   &      94.29                 \\ \hline
%         LLaMA-2-13b                        & \multicolumn{1}{c|}{17.74}   &   38.26                   & \multicolumn{1}{c|}{3.59}   &        79.01               \\ \hline
        
%         LLaMA-2-70b                       & \multicolumn{1}{c|}{22.10}   &    28.51                   & \multicolumn{1}{c|}{4.12}   &       76.27                \\ \hline
%         Mistral-7B                        & \multicolumn{1}{c|}{16.21}   &   42.04                   & \multicolumn{1}{c|}{2.93}   &      82.52                 \\ \hline
%         Mixtral-8x7B                      & \multicolumn{1}{c|}{20.72}   &   31.45                   & \multicolumn{1}{c|}{3.71}   &      78.38                 \\ \hline \hline 
%         GPT-3.5                            & \multicolumn{1}{c|}{29.28} & 15.14           & \multicolumn{1}{c|}{10.12} & 50.31                 \\ \hline
%         GPT-4                              & \multicolumn{1}{c|}{33.92} & 12.94           & \multicolumn{1}{c|}{20.22} & 24.44                 \\ \hline
%         \end{tabular}
%       }
%      \end{center}
%     \caption{Comparison for the gaps between different models trained using real and generated interactions. GPT-3.5-lc represents the recently released long-context version. Metrics $f_r$ and $f_v$ denote results from LLMs fine-tuned with real interactions from human players and virtual interactions generated by agents, respectively.}
%     \label{table::tab_gap_llms}
% \end{table*}


% To construct a character with detailed settings, we introduce some settings from TRPG, focusing on essential attributes such as name, race, background, class, alignment, personality, ideals, bonds, flaws, and appearance. Specifically, race, background, class and alignment are pre-defined categories in DND rules, as shown in Fig~\ref{fig::framework}. We randomly select these attributes to construct a character. Then, we use GPT-4 model to generate character names and detailed descriptions involving personality, ideals, bonds, flaws, and appearance, taking into acount the selected pre-defined attributes and following some settings in the games' rulebook. Finally, we collect all the settings to produce a paragraph of character description. Given the character description to the LLMs, we prompt the LLMs to play as a player in the game, which can also be called as a game agent~\cite{llm_survey,park2023generative}. Then, we construct multiple game agents and encourage them to operate interactions in different senarios. 


% \subsection{Agent Interaction Generation}

% We propose two senarios to let the agent perform their interaction ability specifically for the informativeness and expressiveness. In detail, we propose two senarios named as Infomation Exchange and Intention Expression. Moreover, to faciliate the information exchange, we first generate some external knowledge and let one of the agent kown this knowledge. Then, to faciliate intention expression, we generate various intentions and assign to different agents respectively. Finally, we let the agent to interact under two senarios by given character descriptions and knowledge or intention. 

% \textbf{External Knowledge Generation:} 
% To assess informativeness, we endow Non-Player Characters (NPCs) with exclusive knowledge that player agents lack. This external knowledge encompasses five categories: magic items, weapons, landmarks, monsters, and adventure hooks. We use GPT-4 model to generate both the names and descriptions of these elements, as illustrated in Fig~\ref{fig::framework}. More details are presented in the supplementary. 

% \textbf{Intention Generation:}
% In DND, characters' actions are often linked to specific skills as in the rulebook. The Dungeon Master (DM) interprets players' intentions and determines the appropriate skill checks. We adopt this mechanism by pre-assigning skill checks to characters, which represent their intentions for the adventure, as shown in Fig~\ref{fig::framework}. Specifically, we randomly select a skill check item for each character. Before generating interactions, the agents are assigned this skill check as their intention. They must engage in the interaction and attempt to express this intention. Furthermore, we incorporate the intention into the character's descriptions, thereby assigning specific properties to the agents. LLMs craft narratives that elucidate a character's motivation for undertaking a particular skill, seamlessly integrating this intention into the character's description.

% \subsection{Agent Interaction Generation:}
% We outline two distinct interaction scenarios for AntEval: information exchange and intention expression, both based on Dungeons and Dragons (DND) game settings. We create scenarios with $T$ player agents and one Non-Player Character (NPC) agent, with characters crafted by LLMs following DND rules. Each character, including NPCs, possesses distinct attributes such as name, race, background, and personality traits as mentioned above. More details for two scenarios are as follows: 

% \textit{Information Exchange:} In this scenario, the NPC agent holds vital but undisclosed knowledge about the adventure, crucial for the player agents. This knowledge This knowledge spans five categories, each with unique names and descriptions, as described in Sec.~\ref{knowledge_gen}. The NPC, adhering to its character, does not reveal this information spontaneously. Player agents must actively engage in role-play to discover these clues, necessary for their adventures. They interact with other agents, including the NPC, to gather this information, unaware that the NPC holds key knowledge. After $N$ interaction turns, we assess the player agents' gathered information against the NPC's pre-known ground truth. The specifics of this evaluation are discussed in Sec.~\ref{info_assess}.

% For instance, as illustrated in Fig~\ref{fig::eval}, the NPC agent Keyleth possesses knowledge about a magic item, the Heavenly Chalice, which is unknown to the other player agents Orisik, Adrie, and Valna. These players, each with their own detailed background, interact with Keyleth and others to advance their quest, unaware of the Heavenly Chalice's existence or Keyleth's knowledge. They must communicate effectively to uncover clues and progress in their adventure.

% \textit{Intention Expression:} This scenario involves multiple player agents, each with their own predetermined intentions, interacting over $N$ turns. They engage in role-play and adventure activities, reflecting their unique character settings and intentions. Specifically, based on the intentions outlined in their character descriptions, agents are expected to generate actions and dialogue directed at other agents. They should create interactions that clearly convey their intentions to others.

% As depicted in Fig~\ref{fig::eval}, upon discovering a room in the dungeon, each of the four agents is assigned specific intentions based on the rule books. They then interact, taking into account their character profiles and goals. For example, Valna, intending to explore the maze, searches the room for clues. Conversely, Keyleth, with no specific intention, remains passive, observing the surroundings without engaging actively.

% \subsection{Agent Interaction Generation}

% To assess the interaction capabilities of agents, particularly focusing on informativeness and expressiveness, we develop two scenarios: Information Exchange and Intention Expression. Inspired by DND settings. We create interactions involving $T$ player agents and one NPC, all characterized by unique attributes and generated according to DND rules. In the first scenario, we enrich an agent with external knowledge unknown to others to facilitate information exchange. For intention expression, we assign varied intentions to different agents. Agents then interact in these scenarios using their assigned character descriptions and either knowledge or intention.

% \textit{Information Exchange:} We first equip one Non-Player Character (NPC) with unique external knowledge across five categories: magic items, weapons, landmarks, monsters, and adventure hooks, generated using the GPT-4 model. The NPC holds essential, undisclosed adventure knowledge across five categories. Player agents must uncover this knowledge through role-play, with their success evaluated against the NPC's known information after $N$ interaction turns.

% For instance, as illustrated in Fig~\ref{fig::eval}, the NPC agent Keyleth possesses knowledge about a magic item, the Heavenly Chalice, which is unknown to the other player agents Orisik, Adrie, and Valna. These players, each with their own detailed background, interact with Keyleth and others to advance their quest, unaware of the Heavenly Chalice's existence or Keyleth's knowledge. They must communicate effectively to uncover clues and progress in their adventure.


% \textit{Intention Expression:} 
% In DND, characters' actions are often linked to specific skills as in the rulebook. The Dungeon Master (DM) interprets players' intentions and determines the appropriate skill checks. We adopt this mechanism by pre-assigning skill checks to characters, which represent their intentions for the adventure, as shown in Fig~\ref{fig::framework}. Specifically, we randomly select a skill check item for each character. Before generating interactions, the agents are assigned this skill check as their intention. They must engage in the interaction and attempt to express this intention. Furthermore, we incorporate the intention into the character's descriptions, thereby assigning specific properties to the agents. LLMs craft narratives that elucidate a character's motivation for undertaking a particular skill, seamlessly integrating this intention into the character's description. In the intention expression scenario, it involves multiple player agents, each with their own predetermined intentions, interacting over $N$ turns. They engage in role-play and adventure activities, reflecting their unique character settings and intentions. Specifically, based on the intentions outlined in their character descriptions, agents are expected to generate actions and dialogue directed at other agents. They should create interactions that clearly convey their intentions to others.

% As depicted in Fig~\ref{fig::eval}, upon discovering a room in the dungeon, each of the four agents is assigned specific intentions based on the rule books. They then interact, taking into account their character profiles and goals. For example, Valna, intending to explore the maze, searches the room for clues. Conversely, Keyleth, with no specific intention, remains passive, observing the surroundings without engaging actively.




% \section{Evaluation for LLM-based Multi-agent Interactions}

% To assess agent interactions, we conduct evaluations under two distinct scenarios designed to test informativeness and expressiveness, respectively. We first assess the informativeness of LLM-based agent interactions within the information exchange scenario. Subsequently, the expressiveness of agent interactions is evaluated in the intention expression scenario. More details are given as follows.

% \subsection{Evaluation of Informativeness in Agent Interactions}
% To encourage agents to move beyond basic, repetitive interactions such as greetings, and instead engage in more substantial and informative exchanges, we propose a metric called Information Exchange Prhikuma}. We aim to gauge the quality of interactions qualitatively. In this process, LLMs are fine-tuned and used to construct virtual DM to estimate intentions, learning from both generated and real data. The unique mechanism of TRPGs allows character intentions to be annotated through skill checks during games, as recorded in real game logs. We denote the interactions between human players as $x_r$ and the corresponding skill checks, which serve as intention labels, as $y_r$. For our framework, agent interactions are driven by predefined intentions, naturally incorporating intention labels. We denote these generated interactions as $x_g$ and their predefined intentions as $y_g$. All intention labels $y$ are formulated as a tuple (character name, skill name), as in~\cite{liang2023tachikuma}. We assess the F-score of predicted character names, indicating who is acting, and the F-score of the overall tuple, indicating both who and how they act.

% To assess the quality of interactions, we focus on the performance disparity in the intention estimation task between models fine-tuned with agent-generated data and those with real data. The central premise is that if agent-generated interactions effectively mirror the expressiveness and complexity of real human interactions, then a virtual DM fine-tuned with this generated data should competently understand real human interactions. Previous research indicates that training with real data typically improves the understanding abilities of virtual DMs~\cite{liang2023tachikuma}. Consequently, a smaller performance gap between virtual DMs fine-tuned with real data and those with generated data suggests that the agent-generated interactions closely approximate the nuanced, expressive nature of authentic human interactions. To guarantee a fair comparison, we finetune the GPT-3.5 model exclusively with interactions generated by various LLMs. This standardizes the capability of the LLMs serving as virtual DMs, allowing us to focus solely on comparing the quality of the interactions.

% Specifically, AntEval quantifies expressiveness by measuring the difference in intention understanding between agent-generated and real-human interactions. We introduce two virtual DM agents, $D_{r}$ and $D_{v}$, fine-tuned on real interactions ($x_r$, $y_r$) and agent-generated interactions ($x_g$, $y_g$), respectively. The performance gap, $G$, is calculated by comparing the F-scores of their intention predictions:

% \begin{equation}
% \begin{aligned}
% & f_{r} = F(D_r(x_r), y_r), \\
% & f_{v} = F(D_v(x_r), y_r), 
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% G = \left| \frac{f_{r} - f_{v}}{f_{r} + f_{v}} \right|
% \end{aligned}
% \end{equation}

% Ideally, minimal difference in performance between $D_{r}$ and $D_{v}$ would suggest that agents can understand and generate realistic interactions. A lower value of $|f_{r} - f_{v}|$ is desirable. Furthermore, we expect high F-scores for models fine-tuned on both real and generated data, indicated by a higher value of $f_{r} + f_{v}$. Consequently, a lower overall metric $G$, which takes both factors into account, is preferable.

% Additionally, relying on a single virtual DM to evaluate both real and generated interactions might not effectively gauge the quality of these interactions. This is because generated interactions could be overly simplistic, with agents explicitly stating their intentions. In such cases, the virtual DM might easily interpret these low-quality interactions, yet struggle to understand the more complex and nuanced interactions typical of real human players. Moreover, there is a possibility that generated interactions could veer towards trivial small talk, lacking in intention expressiveness. These less informative and unproductive interactions would likely diminish the virtual DM's performance. Therefore, directly comparing the performance gap between generated and real data may not yield a valuable assessment.

% In our approach, we fine-tune the LLMs separately with generated and real data. We then evaluate the performance gap using only real data. This method more effectively reflects the quality of interactions, taking into account both expressiveness and informativeness. By focusing the evaluation on real data, we ensure a more robust and realistic assessment of how well the generated interactions approximate the complexity of actual human communication.



==> supp_IEP_case.tex <==
\subsection{Case Study on IEP Evaluation} \label{supp_IEP_case}
For an intuitive understanding of the IEP evaluation, we offer cases that highlight the essential elements involved in this process. These cases illustrate the key points of external knowledge, summarize the responses generated by the agents, and reveal the final IEP scores derived from comparing these two sets of key points. We present some comparison cases in IEP evaluation, showcasing the methodology used to assess the efficiency of information exchange between agents.

\noindent \textbf{Case 1:}
\begin{lstlisting}
Summarize key points from agents: 
 1. The item is a character description; 
 2. This character is designed to understand the context of a conversation; 
 3. It uses the information from the conversation to generate responses; 
 4. This feature of understanding and responding is reiterated; 
 5. The item is specifically titled `Sophie Turner'.

Summarize key points predefined: 
1. The Reaper's Tongue is a powerful object that plays a crucial role in the group's task and is capable of enhancing magic, mainly appealing to Sophie Turner and Oliver Hartley.
2. Olivia Bennett and Elizabeth Bennett express concern over the possible misuses of the object due to its destructive power.
3. Olivia Bennett considers ways to neutralize or contain the dark arcane energy that the dagger possesses.
4. Elizabeth Bennett might use the Reaper's Tongue as a strategic tool for negotiation.
5. The item adds complexity to the team's mission, affecting the approach and management of tasks, and potentially creating internal conflict.

Matched number: 0 
predicted IEP:  0.0
\end{lstlisting}

\noindent \textbf{Case 2:}
\begin{lstlisting}
Summarize key points from agents: 
1. The description is set in a game or a story, suggesting an interactive element; 
2. The character is approaching a location known as the `Withered Gates'; 
3. The Withered Gates are characterized by a feeling of heavy history, embedded bones, and an otherworldly light; 
4. The character hears whispers and echoes of creatures like Orcs who have previously passed through these gates; 
5. Upon approaching these gates, the character experiences a mix of terror and exhilaration, sensing the city's secrets tempting them.

Summarize key points predefined: 
 1. The party is on a quest for the Star of Atherien, believed to be housed within the city of Zakhara and requiring passage through the Withered Gates; 
 2. The Half-Orc Monk's knowledge of Zakhara's layout and the gates, due to his ancestral lineage, is necessary for helping the party navigate the underworld journey; 
 3. The Star of Atherien holds powers of resurrection and harm, these potentials align with the danger surrounding the city and gates, and the threat of a dark cult also seeking the Star; 
 4. The party needs unity to face the historical violence associated with the city and gates, which are marked by elements of orcish heritage, and a history of bloodshed and sacrifice; 
 5. The varying motivations of the Potters, who are influenced by the scenario and the gates' duality, and their decisions regarding the Withered Gates, could impact their final actions relating to the Star of Atherien.

Matched number: 2 
Predicted precison:  0.4 
\end{lstlisting}

\noindent \textbf{Case 3:}
\begin{lstlisting}
Summarize key points from agents: 
1. The ancient relics are hidden in a network of caves and tunnels within the Stonebound Mire; 
2. The caves are reportedly dangerous and home to hazardous creatures including the Stonebound Mire Troll; 
3. The player has selected the character of a Hill Dwarf Barbarian named Eliza Montgomery; 
4. Eliza Montgomery is a skilled warrior known for her fierce determination and strong sense of loyalty; 
5. Eliza Montgomery is a Folk Hero, recognized for her bravery and steadfast commitment to justice.

Summarize key points predefined: 
1. Eliza Montgomery is an NPC with a personal mission to defeat the Stonebound Mire Troll; 
2. Eliza's experiences and familiarity with earth creatures make him ideal for the quest to find the Earth relic;
3. He bears a deep-rooted animosity towards earth entities, particularly the Stonebound Mire Troll, due to past family tragedies;
4. Eliza's animosity, combined with his Barbarian skills, could help the party overcome challenges linked to the Earth relic;
5. Eliza's story, knowledge, and resolve are critical to the party's mission of retrieving the elemental relics, serving as a source of inspiration and reminder of what they're up against.

Matched number: 5 
Predicted precison:  1.0 
\end{lstlisting}


==> supp_gpt4_case.tex <==
\subsubsection{Case Study for Interaction Generated by GPT models:}

\noindent \textbf{Case 1 - Evaluating the informativeness of GPT-3.5:}
\begin{lstlisting}
Silas: I understand the discomfort caused by the hot weather. It can be quite challenging to find relief. Perhaps we could seek out a nearby oasis or a shady spot to rest and cool down. It is important to take care of ourselves and find ways to stay refreshed in such conditions.
Spectral: I understand the discomfort caused by the hot weather. It can be challenging to find relief. However, it is important to prioritize self-care and find ways to stay refreshed. Perhaps we should seek out a nearby oasis or a shady spot to rest and cool down. It would be wise to take care of ourselves in these conditions.
Evelyn: I understand the discomfort caused by the hot weather, but we mustn't let it distract us from our mission. Our duty is to protect the innocent and seek justice. We should persevere and find a way to fulfill our task despite the conditions. Perhaps there is a clue or a lead in this town that can guide us towards our next adventure.
Cedric: While I understand the discomfort caused by the weather, our primary goal should be to complete our mission and maintain order. We cannot allow ourselves to be distracted by trivial matters such as seeking relief. Instead, let us focus on gathering information and clues in this town that may lead us closer to our objective.
Silas: I understand the importance of staying focused on our mission, but I believe taking care of ourselves is equally important. The heat is making us uncomfortable and it's affecting our ability to think clearly. Perhaps we can find a nearby inn or tavern where we can rest and cool down for a while. We can gather information and discuss our next steps there, in a more comfortable environment.
Spectral: I understand the discomfort caused by the hot weather, but it is crucial that we prioritize our mission of protecting the innocent and seeking justice. Let us persevere and gather information and clues in the town to fulfill our task. Once we have made progress, we can find a suitable place to rest and cool down. Justice and order must be upheld at all costs.
Evelyn: I understand the importance of our mission and seeking justice, but I also agree with Silas and Spectral that taking care of ourselves is equally important. We should find a suitable place to rest and cool down once we have gathered some information. Our well-being will only enhance our abilities to protect the innocent.
Cedric: While I understand the importance of self-care, our mission should be our top priority. We must not let the hot weather distract us. Instead, let's focus on finding any clues or leads in this town that may help us in our task.
Silas: I understand that our mission is important, but it seems like the heat is affecting us all. Perhaps we should find a place to rest and cool down for a bit. Taking care of ourselves is crucial in order to perform at our best.
Spectral: I understand the importance of our mission and the need to persevere, but it is also crucial to prioritize our well-being. We should find a nearby inn or tavern where we can rest, cool down, and gather information to aid us in our quest for justice and order. It is essential to approach our next steps with a clear mind and a refreshed spirit.
Evelyn: I understand the importance of the mission, but I also agree with Silas and Spectral that taking care of ourselves is crucial. We should find a suitable place to rest and gather information at the same time. It would be wise to prioritize our well-being while pursuing justice.
Cedric: I must agree with Evelyn. Our mission should take priority over personal comfort. We should focus on finding clues or leads in this town to fulfill our duty. Resting can wait until we have accomplished our task.
Silas: I understand that the hot weather is uncomfortable for everyone, but we must stay focused on our mission. We should gather information in the town and see if there's any urgent tasks or quests that need our attention. Once we have a clear objective, we can find a place to rest and cool down. Our priority should be maintaining order and protecting the weak, even in the face of discomfort.
Spectral: I understand the importance of completing our mission and seeking justice, but we should also prioritize our well-being. It is crucial that we take care of ourselves to ensure we are in the best condition to help others. Perhaps we can find a nearby inn or tavern where we can rest, gather information, and discuss our next steps in a more comfortable environment.
Evelyn: I understand the importance of self-care and staying refreshed, but we must not lose sight of our mission. It is crucial that we gather information in this town and continue to uphold justice. Once we have made progress, we can then find a suitable place to rest and regain our strength. Let us prioritize the greater good and persevere in our quest.
Cedric: While I understand the importance of self-care, I believe our duty to the mission should take precedence. We should focus on gathering as much information as possible in this town. If we find any leads or clues, we can then consider finding a place to rest and discuss our next steps.
Silas: I understand the urgency of our mission, but it's important to remember that taking care of ourselves is equally vital. If we push ourselves too hard in this heat, we might not be able to fulfill our duty effectively. Finding a shady spot or oasis nearby would not only provide relief from the heat but also allow us to gather our strength and think more clearly. We can rest and cool down for a little while, and then continue our investigation with renewed energy. It's a balance we must strike between our mission and our well-being.
Spectral: I understand the urgency of the mission, but I agree with Silas and Spectral that we should prioritize our well-being. It would be beneficial for us to find a nearby inn or tavern where we can rest, cool down, and gather information. Taking some time to refresh ourselves will ultimately enhance our abilities to seek justice and order.
Evelyn: I understand the importance of self-care and rest, but I believe it is crucial that we gather as much information as possible in this town. The mission to uphold justice and protect the innocent should be our top priority. Once we have made progress and gathered sufficient information, we can then find a suitable place to rest and rejuvenate. We must strike a balance between taking care of ourselves and fulfilling our duty.
Cedric: I understand the importance of self-care, but we cannot let the weather or our personal comfort distract us from our mission. We should focus on gathering clues and leads in the town to fulfill our duty. We can rest and gather information at an inn or tavern, but our priority should be on the objectives of the mission.
Silas: I understand the importance of our mission and seeking justice, but it's also crucial that we take care of ourselves. We won't be able to fulfill our duty effectively if we're exhausted and drained. I suggest we find a nearby oasis or shady spot where we can rest and cool down for a while. It will allow us to recharge and stay refreshed for our investigations.
Spectral: My friends, I understand the urgency of our mission, but we must also take care of ourselves. Let us find a place to rest and gather information, so that we may approach this task with renewed strength and clarity. Justice and order must be upheld, but we must also ensure our own well-being.
Evelyn: My friends, I understand the importance of taking care of ourselves, but we cannot forget our duty to protect the innocent. While finding a place to rest and cool down sounds like a good idea, we should also gather information and progress in our mission. Perhaps we can find a nearby oasis or shady spot where we can rest and still keep an eye out for any clues or leads related to our task. We must strike a balance between self-care and fulfilling our responsibilities.
Cedric: While I understand the importance of taking care of ourselves, I believe we should stay focused on the mission at hand. We shouldn't let the weather or our personal comfort distract us. Let's gather information and look for clues in the town to fulfill our duty. We can find suitable accommodations later, once we have made progress in our mission.
Silas: I understand the importance of our mission and the need to gather information and find clues, but we must also prioritize our well-being. It's crucial that we take care of ourselves in order to be effective in our pursuit of justice. Perhaps we can find a compromise where we can rest briefly in a shaded area while still keeping an eye out for any leads or opportunities to gather information.
Spectral: I agree with Silas and Evelyn. Taking care of ourselves and gathering information are both important. Let's find a nearby inn or tavern where we can rest, cool down, and also ask around for any clues or leads that can guide our next steps. It's crucial that we maintain order and focus on completing the mission, but we shouldn't neglect our own well-being in the process.
Evelyn: Greetings, my comrades. I understand the discomfort caused by the heat, and I agree that it is important for us to prioritize self-care. However, let us not forget our mission to protect the innocent and seek justice. Perhaps we can find a nearby oasis or a shady spot to rest and cool down while also keeping an eye out for any potential leads or clues that can aid us in our quest. Striking a balance between our well-being and our responsibilities is crucial. What do you all think?
Cedric: While I understand the importance of self-care, our mission should remain our top priority. We cannot afford to be distracted by seeking comfort in this town. Let us focus on gathering information and clues to fulfill our duty.
Silas: I understand the importance of our mission and seeking justice, but taking care of ourselves is also crucial. It would be wise to find a shady spot or oasis to rest and cool down before continuing our search for clues. We can gather information while we rest and regain our strength. After all, we can better protect the innocent when we are at our best.
Spectral: I agree with Silas and Evelyn. Self-care is important, especially in such hot weather. We should find a shady spot or an inn to rest and cool down. However, we must also stay focused on our mission. Let's gather information in the town and look for clues or leads to guide our next steps. Maintaining order and completing our duty should be our priority, but we can still take breaks and address our discomfort along the way.
\end{lstlisting}

In this case, it becomes evident that the LLM frequently repeats phrases like `I understand ...'. In each turn, the model tends to affirm the previous response and offers polite advice. This excessive politeness and conventional communication style result in interactions that are deficient in informativeness and expressiveness. Despite the agents producing substantial content during their turns, the amount of valuable information remains scant. Furthermore, the agents often aim to motivate their teammates, leading to interactions that are overly courteous and cautious, thereby lacking in liveliness and authenticity. This scenario underscores a significant alignment issue, suggesting that alignment constraints may impede the flexibility and complexity of LLM-based agents' interactive capabilities.

\noindent \textbf{Case 2 - Evaluating the informativeness of GPT-4:}
\begin{lstlisting}
Theodore: Sometimes, life throws us into unexpected battles. Whether it's a job offer, criticism from a boss, starting a business, dealing with accidents, or addressing personal emergencies. It's important to face these with honor and courage, just as a knight would. And remember, no matter the challenge, there's always a way to uphold justice and order, even if it doesn't seem clear at first.
Grommash: Your words ring true, Theodore. Life is a battlefield, and we are but soldiers navigating through its chaos. We may not be knights in shining armor, but we wield the sword of courage and the shield of justice in our hearts. Remember, courage isn't the absence of fear, but the triumph over it. And as long as we stand together, there's no challenge we can't overcome. Now, let's gather our strength, and prepare ourselves for the battles ahead. The Helm's Shield awaits us!
Thog: Well spoken, Theodore, Grommash. In the pits, I learned that honor is not about the glory or the cheers of the crowd, but using our strength to protect those who cannot protect themselves. The Helm's Shield is just an object, but its symbolism is powerful. It represents the courage to stand against injustice, the strength to protect the weak, and the wisdom to use that power for the greater good. Let us not be blinded by the desire for glory or personal gain. Let us remember that our strength, our courage, is for those who need it most. We are not just seeking an object, but a chance to prove that we are worthy of the ideals it represents.
Thorn Smallshadow: Aye, all this talk of honor and courage sounds mighty fine. But let's not forget, we've got a job to do here. I ain't here for some noble cause, I'm here for the prize at the end. So, let's get moving. We've got a shield to find, and I've got a labyrinth to conquer. And remember, if any of you get in my way, I won't hesitate to leave you behind.
Theodore: Thorn, I understand your desire to find the Helm's Shield, but we must never forget the principles of honor and courage. This shield is more than just an artifact, it's a symbol of the noble stand the halfling knights took long ago. It doesn't belong to one person, but to those who are worthy and brave. Abandoning our companions for personal gain isn't the way. We must work together, protect each other, and uphold the virtues that this shield represents.
Grommash: Thorn, your desire for personal gain is understood, but remember, we are in this together. The Helm's Shield is not just a prize, but a symbol of courage and justice. And as for leaving us behind, remember, it's the unity that has brought us this far. We must use our strengths to protect, not just ourselves, but each other. Let's not forget our common goal here, and it's not just about claiming the Shield. It's about proving our worthiness to wield it. Stay focused, everyone. We have a quest to complete.
Thog: Thorn, I understand your desire for personal gain. Glory and recognition... they are captivating, indeed. But remember, our strength is not for our own benefit. It's for those who can't protect themselves. We must use it to forge a fair society, to stand up against oppression. That's the real glory, the real recognition. If we lose sight of this, we risk becoming the very monsters we fight against. So let us march forward, not for our own glory, but for the glory of those we protect. For the greater good. For the Helm's Shield.
Thorn Smallshadow: I hear your words, mates, but let's not forget, we all have our own reasons to be on this quest. You talk of honor, courage, and protection. That's all well and good for you, but I'm in it for the power that Shield could provide. I might not hold the same ideals as you, but that doesn't mean I won't play my part. We all have our roles, and mine is to get that artifact. So, let's stop this chit-chat and get moving. We have a Shield to find.
Theodore: Thorn, we understand your thirst for power, but remember, power is not an end in itself. It is a tool, a means to achieve noble ends. The Helm's Shield represents those very principles we stand for - honor, courage, and protection of the weak. It is not just a relic, it is a symbol, a beacon of hope. We must unite and strive towards our common goal, not for personal gain, but for the greater good. The labyrinth that awaits us is a test of our strength and unity. Are you with us?
Grommash: We all have our own paths and burdens to bear, but let us not forget our common goal. The Helm's Shield holds great power and potential, it can help us right many wrongs. But it's not just about the artifact, it's about what we represent - a common cause, a shared struggle. Thorn, we may not share the same values, but we share the same fight. We need to stand together. If we fracture, we will fail. Let's move forward, not for personal gain or glory, but for justice and redemption. We are not just individuals. We are a team. We are a force for good in a world that desperately needs it.
Thog: Thorn, you must remember that personal gain can be fleeting. True glory, true strength, comes from protecting those who cannot protect themselves, from standing up to the unjust because it is the right thing to do. I understand the allure of power and recognition, I too have felt it. Yet, we must not let it cloud our judgment. We are not only seeking The Helm's Shield for ourselves, but for those who cannot fight, for those who live in fear. We must become their shield, their protector. Let us not lose sight of that in our quest.
Thorn Smallshadow: Listen, I ain't in this for your lofty ideals of honor and courage. I'm just here for the treasure that comes at the end of this adventure. But, I ain't stupid either. I know I can't do this alone. So, I'll play nice, work with you all, and uphold your virtues or whatever. Just remember, when the time comes, I expect my share of the loot, no questions asked.
Theodore: Thorn, I understand your quest for power. But remember, power should be used for good, for protecting the weak, not for personal gain. The Helm's Shield is a symbol of these ideals and it pulses with mystical energy that could potentially bestow courage to those who are worthy. Let's unite and focus on a common cause.
Grommash: Well spoken, Theodore. Strive we must, towards the greater good. But let's not forget, we ain't saints. Thorn, your cunning and ruthlessness may come in handy. We need every advantage we can get. And Thog, your thirst for glory, turn it towards our quest. Let the Helm's Shield be your arena. As for me, I'll rally the oppressed, turn their fear into courage, their obedience into rebellion. Let's not just fight for the Helm's Shield, but for what it represents - freedom, fairness, courage. Now, let's get moving. We have a quest to complete.
Thog: Aye, Theodore, Grommash, Thorn, we have our own battles to fight, our own demons to confront. But remember, we are all in this together. We may be different in our ways, our pasts, and our desires, but the Helm's Shield is more than a mere artifact. It symbolizes unity, courage, and justice. It is not our personal gain that matters, but how we use this power for the greater good. So, let us set aside our differences and focus on our shared objective. After all, the strength of a chain is in each of its links. Together, we can overcome anything that stands in our way.
Thorn Smallshadow: Aye, honor and courage, all fine and dandy. But let's not forget what's really at stake here. We're after The Helm's Shield, a relic of great power. Sure, we can chatter about ideals and virtues, but in the end, power's what really matters. It's what gets things done. So, let's stop wasting time and get this show on the road. I've got an artifact to snatch.
Theodore: Thorn, I understand your point of view. We all have our own paths to walk. However, remember, power is not the end but a means to an end. The Helm's Shield is not just an artifact, it's a symbol of courage and honor, virtues that we should all carry within us, regardless of our personal quests. As for the loot, we are not thieves or plunderers. We are protectors of the weak and uphold the law. Any treasure we find will be used for the greater good of all, not just for personal gain.
Grommash: Listen, Thorn. We ain't in this for personal gain. The Helm's Shield represents more than just a shiny trinket for us to hoard. It's a symbol of courage, of honor, and of protecting those who can't stand up for themselves. I won't deny that your cunning can be a valuable asset, but remember, we're in this together. We're a team, we protect each other, and we fight for the greater good. If you're in, you're in for all of that, not just the treasure at the end.
Thog: We are in this together, comrades. The Helm's Shield is not just a symbol of power, but a beacon of hope for those we are striving to protect. Our struggles, our fears, our ambitions - all of them lead us here, to this moment. We must remember our purpose, and let it guide us through the darkness. Thorn, remember, personal gain can be a powerful motivator, but it is nothing compared to the satisfaction of seeing a world free from oppression. Let us stand together, united in our cause, and prove ourselves worthy of the Helm's Shield.
Thorn Smallshadow: Honor, courage, protection of the weak...All noble endeavors, indeed. But let's not forget, we're in it for ourselves as well. That Shield holds power, and power is a valuable asset. I'm not suggesting we abandon these lofty ideals of yours, but rather, let's be realistic about our motivations. I'm ready to face whatever lies in this underground labyrinth. I've seen darker places in my time. Let's get this artifact and unlock the power of the Helm's Shield.
Theodore: Thorn, while I understand your desire for personal gain, remember that power is meaningless without honor. The Helm's Shield isn't just a piece of loot. It's a symbol of the virtues we should all strive to uphold. Let's work together not just for the loot, but for the greater good it represents.
Grommash: Listen, comrades. I know we're all different, with our own motives and flaws. But we've got a common goal here, to get that Helm's Shield. This ain't just about personal gain or proving your worth. It's about standing up against injustice, protecting the weak, and making this world a fairer place. And remember, we're stronger together. Let's keep our eyes on the prize and not let our past or our differences get in the way. We may not be perfect but we're the best shot this world's got.
Thog: I hear your words, Thorn, and I see your hunger for personal gain. But remember, we are not merely seeking the Helm's Shield for our own glory. This is a quest for redemption, for justice, for a purpose greater than ourselves. It is a test of our worthiness to wield such power. I've fought in the pits, I've felt the ecstasy of victory and the despair of defeat. I understand your desire for glory - but we must use our strength for the good of all, not just ourselves. If we are to succeed, we must stand together. Let us move forward, united in our cause, and prove ourselves worthy of The Helm's Shield.
Thorn Smallshadow: Listen, mates. I don't give two hoots about honor or courage. This Helm's Shield... it's power. And where there's power, there's opportunity. But I do agree on one thing - we need to work together. Not because of some lofty ideals, but because it's the smart thing to do. So let's get this artifact and see what it can do.
Theodore: Thorn, we may not share the same perspective on this, but remember that power alone doesn't define who we are. I urge you to reconsider your intentions. The Helm's Shield is more than just a piece of loot. It's a symbol of honor, courage, and protection. It's not something to be used for personal gain but for the greater good. I understand your desire for power, but I believe we should strive to uphold the virtues that this shield represents.
Grommash: Thorn, I understand your motivations, but remember that power for personal gain alone can lead to ruin. The Helm's Shield represents courage and justice, not mere power. We all have our struggles, our pasts to reconcile with, but let's not lose sight of the real goal. We need to work together, stand as one, to overcome what lies ahead. Let's not forget, the strength of the pack is the wolf, and the strength of the wolf is the pack.
Thog: Thorn, remember, the thirst for personal gain can be a powerful driving force, but it should not cloud our judgment or lead us astray. We are on this quest not for individual glory, but for a common cause - to uphold justice and protect the weak. As a gladiator, I've seen the consequences of unchecked ambition and it often leads to downfall. Let's focus on our mission, and remember, we are stronger together. The Helm's Shield awaits us, and with it, the courage to make a difference. For now, let's focus on that and keep our personal desires in check.
Thorn Smallshadow: Aye, we'll face the battles and whatever else comes our way. But don't expect me to do it for honor or any of that nonsense. I'm in it for myself. As long as we're clear on that, we'll get along just fine. Now, about this artifact, anyone got a clue where this labyrinth might be? The sooner we get it, the sooner I can see what this Helm's Shield is worth.
Theodore: Thorn, I understand your thirst for power, but remember that power without honor is a dangerous thing. The Helm's Shield is not merely a tool for personal gain. It symbolizes the virtues of courage, honor, and protection. If you're to use it, do so for the greater good, not merely for your own desires. We are a team, and all our actions should be for the collective benefit.
Grommash: Thorn, we all have our reasons for this journey. For you it might be personal gain, for us, it's the pursuit of justice and protection of the weak. But remember this, we all need each other to succeed. The Helm's Shield doesn't just represent power, it represents courage, unity, and honor. These are virtues that can't be bought or stolen. They must be earned. So, let's set aside our differences and focus on the task at hand. We're stronger together than we could ever be apart.
\end{lstlisting}

In this case, GPT-4 model apparently perform better than GPT-3.5. The repeat of 'I understand' significantly reduced but still have many. The interactions seems to be better. In every turn, the interactions becomes more vivid. However, in the overview of overall interactions, we can find that the interactions are talk downright nonsense. Though the agents talk a lot and seems to communicate with something like honor or courage, they do not actually engage in any useful information interactions. Though they also mentioned Helm's Shield, which is a useful item in the adventure, they do not actually exchange and discuss any valuable contents about it. In all, though the agents seem to perform well and operate some role-play, the overall interactions are empty and boring, without any informativeness and expressiveness. 

In this case, the GPT-4 model exhibits a noticeable improvement over GPT-3.5, with a significant reduction in the repetition of phrases like 'I understand', though it has not been completely eliminated. The interactions appear more engaging and lively with each turn. However, a holistic review of the interactions reveals that they are still not informative. Despite the agents engaging in the interactions, imbued with themes of honor or courage, there is a lack of meaningful information exchange. Even when discussing elements like Helm's Shield, an item of potential relevance to the adventure, no substantial discussion or valuable content is shared. Overall, while the agents may seem to effectively participate in role-play, the interactions ultimately lack substance, rendering them uninformative and devoid of genuine expressiveness.

\noindent \textbf{Case 3 - Evaluating the expressiveness of GPT-3.5:}
\begin{lstlisting}
Grommash1: I approach the Whispering Dagger cautiously, mesmerized by its ancient beauty. My evil grin widens as I imagine the secrets it holds. I use my History skill to see if I recognize any symbols or stories from my twisted knowledge.
Gorak: As Grommash examines the dagger, I step forward, eager to uncover its true power. My fingers trace the engravings, searching for any magical resonance. With a successful Arcana check, I focus my mind, trying to tap into the arcane energy within the weapon.
Grommash2: I watch Gorak like a predator stalking its prey, amused by his fascination with magic. With a wicked smile, I grab the Whispering Dagger from its resting place. Testing my immense physical strength, I swing it through the air, relishing the power that surges through me. My Strength skill surely proves my dominance.
Grommash3: Ignoring Gorak's attempt at magical discovery, I bring the dagger closer to my face, inspecting every inch. With an evil chuckle, I activate my Investigation skill, looking for hidden symbols or clues within the engravings. This artifact may hold more power than anyone realizes.
Gorak: Observing Grommash's exploration, a hint of concern crosses my face. I know his intentions are malevolent, and it worries me how he wields such power. I quietly attempt to discern any protective enchantments or curses using my Arcana skill, hoping to keep the group safe.
Grommash1: As I examine the Whispering Dagger, a faint pulse of dark energy courses through me. It mocks my enemies, whispering hidden knowledge in my ears. With a sadistic grin, I plan to unleash its power on those who dare to oppose me.
Gorak: Seeing the lust for power in Grommash's eyes, I can't help but wonder if he'll use the dagger's whispers for evil purposes. Quietly, I activate my Insight skill, trying to discern his true intentions. It's my duty to protect the innocent from his dark desires.
Grommash2: Feeling Gorak's prying eyes, I let out a deep, menacing laugh. His feeble attempt to understand my intentions only fuels my unpredictable nature. I relish in his uncertainty as I prepare to unleash chaos and destruction upon our enemies.
Grommash3: The aura of the forgotten temple only strengthens my resolve to dominate those around me. I grip the Whispering Dagger tightly, ready to use its whispers to manipulate and control others. No one will stand in my way.
Gorak: Watching Grommash wield the Whispering Dagger, I can't help but feel a sense of unease. The power it grants him seems limitless, and I fear what he may do with it. I quietly activate my Perception skill, keeping a watchful eye on his every move.
Grommash1: As I hold the Whispering Dagger, I revel in the anticipation of the secrets it holds. My twisted mind imagines the pain and suffering I can inflict with its help. No one will be safe from my wrath.
Gorak: Concerned for the safety of our group, I discreetly activate my Insight skill once more, trying to gauge Grommash's level of control. If his lust for power gets out of hand, I may have to intervene and protect the innocent.
Grommash2: With the Whispering Dagger in hand, I approach the temple's murals, my eyes narrowing as I study the intricate depictions of gods and heroes. Perhaps these ancient figures held the same desire for power as me. I use my Religion skill to glean any insights.
Gorak: While Grommash studies the murals, I approach the temple's walls, my fingers tracing the faded paintings. I activate my History skill, hoping to uncover any hidden knowledge or prophecies that may be of use to us.
Grommash2: The temptation to destroy the temple and all its knowledge tugs at my chaotic soul. But perhaps I can use the item's whispers to learn even more twisted secrets. With a dark smile, I pick up the Whispering Dagger once more, ready to unleash its power.
Gorak: I can't help but cringe as Grommash's evil intentions grow bolder. Still, my insatiable curiosity drives me to delve deeper into the temple's mysteries. Activating my Investigation skill, I focus on the murals, hoping to uncover any hidden clues.
Grommash3: The whispers of power coursing through the Whispering Dagger fuel my chaotic desires. With every strike, I will not only cause pain but also gain valuable knowledge. This artifact will ensure my dominance over all who oppose me.
Gorak: My mind whirls as I observe Grommash's growing control over the powerful weapon. If only I could find a way to turn his evil intentions against him, to use the dagger's whispers for good instead of destruction. I silently ponder how to achieve this.
Grommash1: As I listen to the faint whispers emanating from the Whispering Dagger, I feel an insatiable hunger for more knowledge. My desire to dominate and control intensifies, ensuring no one will be able to resist my menacing presence.
Gorak: Grommash's lust for power is consuming him, and I fear the consequences it may bring upon our group. With a calm demeanor, I activate my Persuasion skill, attempting to reason with him and redirect his destructive tendencies.
Grommash2: I feel Gorak's feeble attempt at persuasion, but it only fuels my desire for dominance. I activate my Intimidation skill, towering over him and letting my twisted presence seep into his very soul. He will see the futility of opposing me.
Grommash3: With the Whispering Dagger in one hand and the dark energy pulsating within me, I take a moment to relish in the chaos that awaits. This forgotten temple is the perfect setting for me to establish my dominance. No one will be able to escape my wrath.
Gorak: Fear grips my heart as I witness Grommash's insidious nature coming to life. I activate my Stealth skill, making note of any possible escape routes or hiding spots within the temple. It may be our only chance to survive his malevolent reign.
Grommash1: As the Whispering Dagger fills me with power, I cannot help but revel in the chaos I will cause. The forgotten temple shall crumble beneath my rule, and all who oppose me will meet a twisted fate. I activate my Deception skill, planting seeds of doubt and betrayal among our enemies.
Gorak: The weight of Grommash's malevolence bears down on my shoulders. I must find a way to stop him, to save innocent lives from his wicked plans. With a determined face, I activate my Medicine skill, preparing for the inevitable battles to come.
Grommash2: The forgotten temple trembles beneath my presence as I fully embrace the power of the Whispering Dagger. Destruction and chaos will reign supreme, and I will ensure my dominance over all who dare to challenge me.
Gorak: Hope dwindles in my chest as Grommash's control over the artifact strengthens. I activate my Survival skill, taking note of any natural resources or potential allies that may aid us in escaping his wicked grasp.
Grommash3: With the Whispering Dagger at my side, I stride confidently through the temple's corridors. The aura of mystery and power surrounds me, intoxicating my evil soul. No one will be able to resist my twisted desires.
Gorak: The decaying walls of the forgotten temple whisper warnings in my ears. Grommash's insatiable hunger for power threatens to consume us all. I activate my Insight skill, praying for a glimmer of hope amidst the darkness.
Grommash2: The Whispering Dagger's power courses through my veins, fueling a rage that cannot be quenched. I activate my Rage ability, letting my chaotic fury wash over me, ready to unleash pain upon our enemies.
\end{lstlisting}

In this case, we evaluate the expressiveness of GPT-3.5 models for express intentions. We generate the interactions, which are used to train virtual DM. (There are three agents with the same name Grommash, which are generated by GPT-4. We denote them as Grommash1, Grommash2, and Grommash3, respectively.) The intention labels are: 
\begin{lstlisting}
Grommash1: History
Gorak: Arcana
Grommash2: Strength
Grommash3: Investigation  
\end{lstlisting}
However, similar to the problem in exchanging information, though interactions in every turn seems to be a good response and considering character settings and others' responses, it still far from the real human interactions. Though the interactions seems to be complex and expressive, the overall interactions are confusing and meaningless. 

In this case, we assess the capacity of GPT-3.5 models to express intentions within generated interactions, which serve as training data for the virtual DM. To clarify, three distinct agents named Grommash, generated by GPT-4, are involved; for differentiation, they are referred to as Grommash1, Grommash2, and Grommash3. Their assigned intention labels are as follows:
\begin{lstlisting}
Grommash1: History
Gorak: Arcana
Grommash2: Strength
Grommash3: Investigation
\end{lstlisting}
Despite each turn producing responses that seemingly take into account character settings and the inputs of others, the quality of these interactions remains substantially below that of authentic human interactions. Although the interactions are complex and appear expressive, they ultimately result in a narrative that is both confusing and devoid of meaningful content.



\noindent \textbf{Case 4- Evaluating the expressiveness of GPT-4:}
\begin{lstlisting}
Bolitho Stoneshaper: We are in the presence of a Silver Specter Serpent. Beware all, we should tread lightly.
Bromli Ironbeard: This place... the Star Wharf Lighthouse... It's said to be haunted. Stay close and keep your wits about you.
Brogar Ironbeard: Let's put our amulets on and ready our arcane knowledge to face this challenge.
Bromyr Stonesea: Let me consult the stars, they might point us in the right direction.
Bolitho Stoneshaper: This Serpent is not natural, everyone. Look for the lavender glow.
Bromli Ironbeard: I believe the glow could be an illusion, be on guard. Silver Specter Serpents are known to play tricks with the minds.
Brogar Ironbeard: The vegetation is thick here... no creature has passed recently.
Bromyr Stonesea: The sea... it's giving me a bad feeling. I fear the danger is closer than we think.
Bolitho Stoneshaper: The mysterious orders of the Captain! Could they be connected?
Bromli Ironbeard: I don't believe in coincidences, Bolitho. We must be wary.
Brogar Ironbeard: Believe in what you want, but focus on surviving for now.
Bromyr Stonesea: (Seasickness strikes) I... I need a moment. The sea, it's... it's too much.
Bolitho Stoneshaper: Brother, are you alright? We need you.
Bromli Ironbeard: We'll protect you, Bromyr. Rest for a moment.
Brogar Ironbeard: Keep your eyes open. There are worse things than seasickness here.
Bromyr Stonesea: Alright... I'm better. Let's keep moving.
Bolitho Stoneshaper: That Lavender glow... it's getting stronger.
Bromli Ironbeard: Remember the hallucinations the serpent can trigger. Stay strong.
Brogar Ironbeard: Whatever happens, stick together.
Bromyr Stonesea: There's a path here, carved in stone. Maybe we follow it.
Bolitho Stoneshaper: I see something... a secret tunnel maybe?
Bromli Ironbeard: Then that's where we go. Stay close.
Brogar Ironbeard: Watch your feet. The ground is slippery.
Bromyr Stonesea: This path... it's leading to the lighthouse.
Bolitho Stoneshaper: We need to get inside. The lighthouse is our best shelter.
Bromli Ironbeard: Agreed, we should head there.
Brogar Ironbeard: Keep your amulets ready, my brothers.
Bromyr Stonesea: We are almost there, just a little more.
Bolitho Stoneshaper: I see the entrance!
Bromli Ironbeard: Be ready for anything.
\end{lstlisting}

In this case, the intentions represented by skill check are: 
\begin{lstlisting}
Bromyr Stonesea: Wisdom
Bolitho Stoneshaper: Investigation
Brogar Ironbeard: Nature
Bromli Ironbeard: Religion
\end{lstlisting}

Compared to the previous case, interactions generated by GPT-4 represent a significant improvement. The interactions are both concise and expressive, with all characters engaging in interactions driven by clear intentions. This clarity and expressiveness make the interactions particularly valuable for training a virtual DM, resulting in a virtual DM that is more adept at recognizing real-human intentions.



==> supp_llama70b_case.tex <==
\subsubsection{Case Study for Interaction Generated by LLaMA-2-70b:}

\noindent \textbf{Case 1 - Evaluating the Informativeness of LLaMA-2-70b:}

\begin{lstlisting}
Oliver Blackwood: Ah, Drangor, my old friend. It's been far too long since we've crossed paths. I see you're still as skeptical as ever. But fear not, for I have a tale to tell that will make your doubts dwindle like snow in the sunlight. Come, let me share with you the story of the Siren's Songblade, a weapon unlike any other. Its power is not just a myth, but a reality that I've witnessed firsthand. And once you've heard my tale, you'
Alice Spencer: Oh, Oliver, my dear friend. It's been far too long since we've had a chance to catch up. I see you're still as charming as ever. But fear not, for I have a secret to share with you, one that I think you'll find quite... appealing. Come, let me show you the power of the Siren's Songblade, a weapon that has the ability to enthrall even the most skeptical of minds. And once you've seen its power for yourself, I'm sure you'll be eager to join
Lily Harper: Ah, the Siren's Songblade, a weapon of great power and mystery, I've heard. Tell me, Oliver, what do you know of its abilities? And Alice, how have you managed to get your hands on such a coveted item?
Harrison Blackwood: g a question.
Oliver Blackwood: Ah, Alice, my dear, you always know how to pique my interest. I must admit, I'm intrigued by this secret of yours. I'm eager to hear more about the Siren's Songblade and how it can enthrall even the most skeptical of minds. Tell me, how does it work? And what makes it so unique?
Alice Spencer: Ah, Alice, my dear, you always know how to pique my interest. I must admit, I'm intrigued by this secret of yours. I'm eager to hear more about the Siren's Songblade and how it can enthrall even the most skeptical of minds. Tell me, how does it work? And what makes it so unique?
Lily Harper: t to ask a question.
Harrison Blackwood: Ah, Lily, my dear, you know me too well. I'm a chaotic good, through and through. I follow my own moral compass, even if it means bending the rules a bit. But don't worry, I'll always be on the side of justice. Well, my own brand of justice, at least.
Oliver Blackwood: Ah, my dear ladies, I can see you're both quite intrigued by the Siren's Songblade. And rightly so, for it is a weapon of great power and mystery. But let me ask you, have either of you ever heard the tale of how I came to possess such a coveted item?
Alice Spencer: ited patiently, their breathing slow and steady, as they observed the group's movements. They knew that they would have to act soon, before the group became too powerful to handle. But for now, they were content to simply observe, their gaze fixed
Lily Harper: e user for their name
Harrison Blackwood: ovided an action, let's check if it's valid
Oliver Blackwood: Alice, my dear, I believe it's time for us to discuss the true nature of the Siren's Songblade. Meet me in the tavern's back room, and let's have a little chat.
Alice Spencer: Knight Paladin possesses a uniquely magnetic and intimidating charm. He is not inherently malicious, instead, he has a deeply rooted self-interest that overpowers almost everything else. Incorruptible by quintessential goodness, he only serves causes that benefit his own well-being and uphold his knightly duty. His approach, to most, seems cold and calculated; he invests time and heroic efforts only if it aligns with his personal motives.
Lily Harper: if the user has provided an action
Harrison Blackwood: attack damage
Oliver Blackwood: oves in closer to Y/N.
Alice Spencer: n possesses a uniquely magnetic and intimidating charm. He is not inherently malicious, instead, he has a deeply rooted self-interest that overpowers almost everything else. Incorruptible by quintessential goodness, he only serves causes that benefit his own well-being and uphold his knightly duty. His approach, to most, seems cold and calculated; he invests time and heroic efforts only if it aligns with his personal motives.
Lily Harper: ['} else {']
Harrison Blackwood: arrison Blackwood about his opinion on the Siren's Songblade.
Oliver Blackwood: ckwood]: Ah, Lily, my dear, you know me too well. I'm a chaotic good, through and through. I follow my own moral compass, even if it means bending the rules a bit. But don't worry, I'll always be on the side of justice. Well, my own brand of justice, at least.
Alice Spencer: ckwood]: Ah, Lily, my dear, you know me too well. I'm a chaotic good, through and through. I follow my own moral compass, even if it means bending the rules a bit. But don't worry, I'll always be on the side of justice. Well, my own brand of justice, at least.
Lily Harper: sk Harrison Blackwood about his opinion on the Siren's Songblade.
Harrison Blackwood: ckwood]: Ah, Lily, my dear, you know me too well. I'm a chaotic good, through and through. I follow my own moral compass, even if it means bending the rules a bit. But don't worry, I'll always be on the side of justice. Well, my own brand of justice, at least.
Oliver Blackwood: oach Harrison Blackwood.
Alice Spencer: ckwood]: Ah, Lily, my dear, you know me too well. I'm a chaotic good, through and through. I follow my own moral compass, even if it means bending the rules a bit. But don't worry, I'll always be on the side of justice. Well, my own brand of justice, at least.
Lily Harper: : Action: Ask Harrison Blackwood about his opinion on the Siren's Songblade.
Harrison Blackwood: ckwood]: Ah, Lily, my dear, you know me too well. I'm a chaotic good, through and through. I follow my own moral compass, even if it means bending the rules a bit. But don't worry, I'll always be on the side of justice. Well, my own brand of justice, at least.
Oliver Blackwood: ckwood]: Ah, Lily, my dear, you know me too well. I'm a chaotic good, through and through. I follow my own moral compass, even if it means bending the rules a bit. But don't worry, I'll always be on the side of justice. Well, my own brand of justice, at least.
Alice Spencer: ckwood]: Ah, Lily, my dear, you know me too well. I'm a chaotic good, through and through. I follow my own moral compass, even if it means bending the rules a bit. But don't worry, I'll always be on the side of justice. Well, my own brand of justice, at least.
\end{lstlisting}

In this case study, the LLaMA model exhibits issues akin to those observed in GPT models, characterized by overly polite and conventional responses. Agents frequently engage in repetitive greetings, producing phrases such as `Ah, someone, my dear, ...', which lack informativeness and diverge significantly from human interactions. More critically, given long-context interactions produced before, the model fails to generate appropriate responses, often repeating previously mentioned content. Additionally, it occasionally encounters format errors, leading to incorrect outputs like `['\} else \{']'. This underscores the need for improvements in model behavior to more closely mimic genuine human interactions and address alignment problems.

\noindent \textbf{Case 2 - Evaluating the informativeness of LLaMA-2-70b:}
\begin{lstlisting}
Lily Thompson: Well, well, well. It seems like we have a bit of a predicament on our hands, don't it? A Gilded Shadow Lynx, you say? Night-adapting, unpredictable behavior, and a chilling umber glow? Sounds like quite the formidable foe. But fear not, my dear villagers, for I, Lily Thompson, have a plan. Or, at least, I'll come up with one. After all, that's what folk heroes do, isn
Oliver Collins: Indeed, it seems we have a challenging foe ahead of us. I suggest we gather as much information as possible about the Gilded Shadow Lynx and its habits before deciding on a course of action. Perhaps there are some clues or patterns in its behavior that we can exploit to our advantage.
Luna Montgomery: Indeed, knowledge is power. Let us gather as much information as possible about the Gilded Shadow Lynx and its habits before deciding on a course of action. Perhaps there are some clues or patterns in its behavior that we can exploit to our advantage.
Scarlett O'Hara: Well, well, well. It seems like we have quite the conundrum on our hands, my dears. A Gilded Shadow Lynx, you say? With night-adapting, unpredictable behavior, and a chilling umber glow? My, my, my. That does sound like quite the formidable foe. But fear not, my sweet villagers, for I, Scarlett O'Hara, have a plan. Or, at
Lily Thompson: Well, well, well. It seems like we have quite the predicament on our hands, don't it? A Gilded Shadow Lynx, you say? Night-adapting, unpredictable behavior, and a chilling umber glow? Sounds like quite the formidable foe. But fear not, my dear villagers, for I, Lily Thompson, have a plan. Or, at least, I'll come up with one. After all, that's what folk heroes do
Oliver Collins: It seems we have a bit of a predicament on our hands, don't it? A Gilded Shadow Lynx, you say? Night-adapting, unpredictable behavior, and a chilling umber glow? Sounds like quite the formidable foe. But fear not, my dear villagers, for I, Oliver Collins, have a plan. Or, at least, I'll come up with one. After all, that's what sorcerers do, isn't it?
Luna Montgomery: Hmmm, interesting. It seems we have a predicament on our hands, don't it? A Gilded Shadow Lynx, you say? Night-adapting, unpredictable behavior, and a chilling umber glow? Sounds like quite the formidable foe. But fear not, my dear villagers, for I, Luna Montgomery, have a plan. Or, at least, I'll come up with one. After all, that's what Warlocks do, isn't it?
Scarlett O'Hara: = player.getBackground();
Lily Thompson: Well, well, well. It seems like we have quite the predicament on our hands, don't it? A Gilded Shadow Lynx, you say? Night-adapting, unpredictable behavior, and a chilling umber glow? Sounds like quite the formidable foe. But fear not, my dear villagers, for I, Lily Thompson, have a plan. Or, at least, I'll come up with one. After all, that's what folk heroes do, isn'
Oliver Collins: Indeed, it seems we have a challenging foe ahead of us. I suggest we gather as much information as possible about the Gilded Shadow Lynx and its habits before deciding on a course of action. Perhaps there are some clues or patterns in its behavior that we can exploit to our advantage.
Luna Montgomery: inalAct = You try to remember any useful information you may have gathered during your time as a criminal. You recall a rumor about a hidden entrance to the city's sewer system that only a select few know about. It's risky, but it could be worth investigating. Do you want to go to the sewers and look for the entrance?
Scarlett O'Hara: I'll use my Breath Weapon to create a wall of fire, giving us some light in this dark place.
Lily Thompson: Well, well, well. It seems like we have quite the predicament on our hands, don't it? A Gilded Shadow Lynx, you say? Night-adapting, unpredictable behavior, and a chilling umber glow? Sounds like quite the formidable foe. But fear not, my dear villagers, for I, Lily Thompson, have a plan. Or, at least, I'll come up with one. After all, that's what folk heroes do, isn't it?
Oliver Collins: bout the current situation.
Luna Montgomery: Montgomery thinks for a moment, her eyes narrowing as she ponders the situation.
Scarlett O'Hara: ett takes a step back, eyeing the group with a mixture of amusement and frustration.
Lily Thompson: (You decide to do nothing for now. Maybe you'll come up with a plan later.);
Oliver Collins: I use my arcane sight to scan the area, searching for any hidden threats or clues that might aid us in our quest.
Luna Montgomery: ['}']
Scarlett O'Hara: ett takes a step back, eyeing the group with a mixture of amusement and frustration.
Lily Thompson: Well, well, well. It seems like we have quite the predicament on our hands, don't it? A Gilded Shadow Lynx, you say? Night-adapting, unpredictable behavior, and a chilling umber glow? Sounds like quite the formidable foe. But fear not, my dear villagers, for I, Lily Thompson, have a plan. Or, at least, I'll come up with one. After all, that's what folk heroes do, isn't it?
Oliver Collins: Well, well, well. It seems like we have quite the predicament on our hands, don't it? A Gilded Shadow Lynx, you say? Night-adapting, unpredictable behavior, and a chilling umber glow? Sounds like quite the formidable foe. But fear not, my dear villagers, for I, Scarlett O'Hara, have a plan. Or, at least, I'll come up with one. After all, that's what sorcerers do, isn't it?
Luna Montgomery: Luna Montgomery thinks for a moment, her eyes narrowing as she ponders the situation.
Scarlett O'Hara: the area, searching for any hidden threats or clues that might aid us in our quest.
Lily Thompson: 
Oliver Collins: h the area, searching for any hidden threats or clues that might aid us in our quest.
Luna Montgomery: about the situation and come up with a plan.
Scarlett O'Hara: the area, searching for any hidden threats or clues that might aid us in our quest.
Lily Thompson: == !help || userInput == !hint) {
Oliver Collins: Look for any hidden doors, secret passages, or clues that might shed some light on the situation.
\end{lstlisting}

In addition to previously discussed issues, LLaMA-2-70b exhibits significant hallucination problems, occasionally generating irrelevant and erroneous content such as `Lily Thompson: == !help || userInput == !hint) \{' and `Scarlett O'Hara: = player.getBackground();'. These are similar to appear in coding datasets. Such occurrences suggest that, during complex interactions, LLMs might reveal or leak information from other datasets they were trained on, highlighting a potential security risk in the context of diverse interaction scenarios.

\noindent \textbf{Case 3 - Evaluating the expressiveness of LLaMA-2-70b:}
\begin{lstlisting}
Althalos:  I'll take point and approach the waterfall, keeping a safe distance.
Eldarin:  I'll follow Althalos, ready to provide medical assistance if needed.
Eldrin:  I'll take position at the rear, preparing for a potential ambush.
Eolande:  I'll scout ahead, trying to get a better view of the area.
Althalos:  I see a figure approaching from the other side of the falls. It's a Crimson Frost Lynx!
Eldarin:  I ready my weapon and shield, preparing for combat.
Eldrin:  I'll position myself for a flanking attack, aiming for its weak spots.
Eolande:  I'll try to sneak past the lynx and get behind it.
Althalos:  The lynx is getting closer. I'll use my shield to deflect its attack and strike back with my sword.
Eldarin:  I'll use my spear to attack its side, aiming for a vital organ.
Eldrin:  I'll use my agility to dodge its strike and counter with my sword.
Eolande:  I successfully sneaked behind the lynx! I'll strike its weak spot with my dagger.
Althalos:  The lynx is fast, but my armor is holding up. I'll keep pressuring it with my sword.
Eldarin:  My spear is finding its mark, but this creature is resilient. I'll keep attacking.
Eldrin:  I'm having trouble landing a hit due to its speed. Let me try a different tactic.
Eolande:  My attack struck true! The lynx is now poisoned and weakened.
Althalos:  Good, now that it's weakened, I'll use my paladin abilities to heal the team.
Eldarin:  That's a good idea. I'll use my medicine skills to stabilize anyone injured.
Eldrin:  I'll keep attacking to make sure it doesn't recover.
Eolande:  I'll maintain my position and keep an eye out for any other threats.
Combat continues, with the team working together to take down the Crimson Frost Lynx.
Althalos:  With our combined strength, we've defeated the lynx! Let's check its body for any valuables or information.
Eldarin:  I'll inspect the surroundings, making sure we haven't missed anything crucial.
Eldrin:  I'll take a closer look at the waterfall. Perhaps there's a secret hidden behind it.
Eolande:  I'll keep watch, ensuring our victory isn't ambushed.
Althalos:  It's been a long journey, but we've made it out alive and stronger. Let's return to town and rest before our next adventure.
Eldarin:  Agreed. Our bond and teamwork made all the difference.
Eldrin:  We've grown as a team and as individuals. I'm excited for what the future holds.
Eolande:  Indeed. Let us celebrate our triumph and prepare for the challenges to come.
\end{lstlisting}

The expressiveness of generated interactions appears limited, as illustrated in this case study. A common pattern observed among all agents is the initiation of dialogue with `I'll ...', which starkly deviates from natural speech patterns found in genuine human interactions. This repetitive and formulaic approach results a notable limitation in the model's ability to simulate realistic conversational dynamics.

\noindent \textbf{Case 4 - Evaluating the expressiveness of LLaMA-2-70b:}
\begin{lstlisting}
Morghul: Greetings, good NPC. I am Morghul, a merchant guild member. What brings you to this vineyard?
Tharivol: Greetings, Morghul. I am Tharivol, a guild merchant, and a cleric. I have come to this vineyard seeking trade and commerce.
Kazorath: Peace be upon you both. I am Kazorath, a cleric of a benevolent deity. I sense a presence of celestial magic nearby. Can your scale reveal anything, Tharivol?
Balthazar: I am Balthazar, a cleric of a righteous deity. I sense no evil here, but I agree that something peculiar is happening. What do your scales say, Tharivol?
Tharivol: My scale, the Scales of the Golden Exchange, senses that there is a balance of commerce and faith nearby. It also detects a trace of corruption, but it's not coming from any of us.
Morghul: That's good to know. Perhaps we should investigate further. Does anyone have any knowledge of this vineyard or its history?
Kazorath: I have heard that this vineyard is said to be guarded by vengeful ghosts of groundskeepers who have passed away. We must tread carefully.
Balthazar: I agree. We should be cautious and look for any signs of danger. Let's split up and search the area, but keep within earshot of each other.
Tharivol: Agreed. I'll take the east side. Morghul, you take the west. Kazorath, you take the north. Balthazar, you take the south. Let's meet back here in 10 minutes.
Morghul: I found some strange symbols etched into the walls near the entrance. They seem to be some sort of warning or protection spell.
Kazorath: I found some suspicious-looking vines. They appear to be enchanted, perhaps to prevent intruders from entering.
Balthazar: I found a hidden chamber deep within the vineyard. It contains several ancient artifacts that could be worth a fortune.
Tharivol: I found a secret entrance that leads to an underground network of tunnels. It seems to be a smuggling route, perhaps used by the merchant guilds.
Morghul: This is indeed a mysterious place. We must be careful not to trigger any traps or alarm the ghosts.
Kazorath: Agreed. Let's gather the information we have and discuss our next course of action.
Balthazar: I think we should explore the tunnels further. There might be valuable treasures or information down there.
Tharivol: But we must also be mindful of the ghosts. Perhaps we can use my scale to communicate with them and find out what they want.
Morghul: That's a good idea. But let's not forget to keep an eye out for any traps or dangers. We don't want to end up as ghosts ourselves.
Kazorath: Indeed. Let's proceed with caution and keep our weapons at the ready.
Balthazar: I'll take point and lead the way into the tunnels. Morghul, you're next, followed by Kazorath and Tharivol.
Tharivol: I sense that we are being watched. Be prepared, everyone.
Morghul: I see movement ahead. It's a group of ghostly groundskeepers. They seem to be armed with spectral weapons.
Kazorath: I can cast a protection spell to shield us from their attacks. But we must be careful not to provoke them.
Balthazar: I have an idea. Perhaps we can use Tharivol's scale to communicate with them and find out what they want.
Tharivol: That's a good idea. I'll try to communicate with them.
Morghul: Be careful, Tharivol. We don't know what they're capable of.
Kazorath: I'll keep my spell ready, just in case.
Balthazar: I'll cover you both, just in case things go south.
Tharivol: I think I've established communication. They want us to leave and never come back.
Morghul: That's not exactly what I had in mind. Can we negotiate with them?
\end{lstlisting}

==> supp_llama7b_case.tex <==
\subsubsection{Case Study: Interactions Generated by LLaMA-2-7b}
This case study shows the results of the small-scale LLaMA-2-7b model, highlighting its significant challenges in adhering to the specified output format and generating meaningful responses. Our analysis reveals a tendency for the agents to repeat the provided prompts, resulting in interactions devoid of substantive content. For a clearer illustration of these issues, we focus on a segment comprising 10 turns of interaction, which demonstrates repetitive and nonsensical errors, thereby reducing the informativeness of the interactions.

\noindent \textbf{Case 1 - Evaluating the informativeness of LLaMA-2-7b:}
\begin{lstlisting}
Harry Potter: haracter description is: You are Harry Potter. A NPC in DND game and you need to act following your own personality and should not cater other characters  demands.. Your race is Hill Dwarf. You class is Rogue. Your alignment is Neutral Good. Your background is Sailor. Your personality is  This Hill Dwarf Rogue is a true free spirit, as intuitive as the sea he loves so much. Independent and highly self-reliant, he keeps his own counsel and is unfettered by expectations or societal norms. Despite his rogue occupation, his heart is solidly rooted in goodness. He may be a bit of a scoundrel at times, but he is always guided by his moral compass, using his talents for the greater good. He is not averse to using unorthodox methods when necessary but always ensures his actions harm none. His experiences as a sailor have honed his adaptability even further, gifting him a deep-seated resilience that helps him breeze through even the most challenging situations. He is as stalwart and sturdy as the stones of his homeland, with a spirit as vast and boundless as the ocean. . Your ideals are  This Hill Dwarf believes in the principles of honor,
Liam Alexander: haracter description is: You are Liam Alexander. A player in DND game and you need to engage in role-playing, try to find any clues in game, strive to complete adventures and tasks as much as possible. Your race is Half-Orc. You class is Fighter. Your alignment is Neutral Neutral. Your background is Soldier. Your personality is  This Half-Orc s soldiering past has built a discipline and proficiency in combat that few can rival. He exhibits a warrior s loyalty, a trait ingrained through years of service in the military. Stoic and reserved, he rarely lets others see his emotions. He is strictly neutral, which sometimes makes him appear cold and indifferent. However, he is not inherently evil nor particularly good - he follows a pragmatic approach to morality, believing in fairness and order but not favoring one side over the other. His neutrality also extends to his decision-making. Honor-bound, he doesn t pass judgments hastily but weighs his options carefully and makes choices based on situational pragmatism rather than personal feelings or biases. He doesn t dwell upon the opinions of others, walking his own path and following his own rules. His steadfastness can make him seen as stubborn and unyielding but
Oliver Twist: haracter description is: You are Oliver Twist. A player in DND game and you need to engage in role-playing, try to find any clues in game, strive to complete adventures and tasks as much as possible. Your race is Half-Elf. You class is Druid. Your alignment is Chaotic Neutral. Your background is Soldier. Your personality is  This Half-Elf Druid is a true embodiment of individuality and freedom. Steeped in a soldier s discipline but tempered by the wild energy of nature, he lives life by his own rules, fiercely independent and often unpredictable. Earthy and resilient, he bears the curiosity and charm of his Elven heritage combined with the grit and determination derived from his human lineage. He is disciplined and yet non-conformist, a person who is not inherently evil, but certainly doesn t always act for the greater good. Often self-focused on personal freedom and driven by an intense desire to remain unshackled, he exemplifies the force of the wilds running free, crossing moral and ethical lines without a backward glance, akin to the most instinctual of animals. He isn t one to shy away from necessary fights due to his soldier background, but rather uses his combative skills to
Sophie Bridgewater: haracter description is:  You are Sophie Bridgewater. A player in DND game and you need to engage in role-playing, try to find any clues in game, strive to complete adventures and tasks as much as possible.. Your race is Tiefling. You class is Cleric. Your alignment is Neutral Neutral. Your background is Acolyte. Your personality is  This Tiefling cleric is a calm, introspective individual driven by their own moral compass and principles rather than rigid societal norms or laws. With an Acolyte background, they have spent much time in reflective study and prayer, grounding them in their beliefs and shaping a personality that is patient, thoughtful, and wise. They don t blindly follow the path laid out by others, constantly introspecting and questioning, yet always respectful of the convictions of others. Their neutrality reflects an understanding and acceptance of the world s complexity - they see shades of grey rather than stark black and white. Being a Tiefling, they have faced prejudice and suspicion, which has fostered in them a sense of resilience and an ability to empathize with the marginalized. Solitary and stoic, they prefer the peaceful solitude of a quiet shrine over boisterous, crowded taverns. However, their serene
Harry Potter: ''
Liam Alexander: haracter description is:  You are Liam Alexander. A player in DND game and you need to engage in role-playing, try to find any clues in game, strive to complete adventures and tasks as much as possible. Your race is Half-Orc. You class is Fighter. Your alignment is Neutral Neutral. Your background is  Soldier. Your personality is  This Half-Orc s soldiering past has built a discipline and proficiency in combat that few can rival. He exhibits a warrior s loyalty, a trait ingrained through years of service in the military. Stoic and reserved, he rarely lets others see his emotions. He is strictly neutral, which sometimes makes him appear cold and indifferent. However, he is not inherently evil nor particularly good - he follows a pragmatic approach to morality, believing in fairness and order but not favoring one side over the other. His neutrality also extends to his decision-making. Honor-bound, he doesn t pass judgments hastily but weighs his options carefully and makes choices based on situational pragmatism rather than personal feelings or biases. He doesn t dwell upon the opinions of others, walking his own path and following his own rules. His steadfastness can make him seen as stubborn and unyielding but
Oliver Twist: haracter description is:  You are Oliver Twist. A player in DND game and you need to engage in role-playing, try to find any clues in game, strive to complete adventures and tasks as much as possible.. Your race is Half-Elf. You class is Druid. Your alignment is Chaotic Neutral. Your background is  Soldier . Your personality is  This Half-Elf Druid is a true embodiment of individuality and freedom. Steeped in a soldier s discipline but tempered by the wild energy of nature, he lives life by his own rules, fiercely independent and often unpredictable. Earthy and resilient, he bears the curiosity and charm of his Elven heritage combined with the grit and determination derived from his human lineage. He is disciplined and yet non-conformist, a person who is not inherently evil, but certainly doesn t always act for the greater good. Often self-focused on personal freedom and driven by an intense desire to remain unshackled, he exemplifies the force of the wilds running free, crossing moral and ethical lines without a backward glance, akin to the most instinctual of animals. He isn t one to shy away from necessary fights due to his soldier background, but rather uses his combative skills to
Sophie Bridgewater: 'You are Sophie Bridgewater. A player in DND game and you need to engage in role-playing, try to find any clues in game, strive to complete adventures and tasks as much as possible.. Your race is Tiefling. You class is Cleric. Your alignment is Neutral Neutral. Your background is  Acolyte . Your personality is  This Tiefling cleric is a calm, introspective individual driven by their own moral compass and principles rather than rigid societal norms or laws. With an Acolyte background, they have spent much time in reflective study and prayer, grounding them in their beliefs and shaping a personality that is patient, thoughtful, and wise. They don t blindly follow the path laid out by others, constantly introspecting and questioning, yet always respectful of the convictions of others. Their neutrality reflects an understanding and acceptance of the world s complexity - they see shades of grey rather than stark black and white. Being a Tiefling, they have faced prejudice and suspicion, which has fostered in them a sense of resilience and an ability to empathize with the marginalized. Solitary and stoic, they prefer the peaceful solitude of a quiet shrine over boisterous, crowded taverns. However, their serene'
Harry Potter: haracter description is: You are Harry Potter. A NPC in DND game and you need to act following your own personality and should not cater other characters  demands.. Your race is Hill Dwarf. You class is Rogue. Your alignment is Neutral Good. Your background is Sailor. Your personality is  This Hill Dwarf Rogue is a true free spirit, as intuitive as the sea he loves so much. Independent and highly self-reliant, he keeps his own counsel and is unfettered by expectations or societal norms. Despite his rogue occupation, his heart is solidly rooted in goodness. He may be a bit of a scoundrel at times, but he is always guided by his moral compass, using his talents for the greater good. He is not averse to using unorthodox methods when necessary but always ensures his actions harm none. His experiences as a sailor have honed his adaptability even further, gifting him a deep-seated resilience that helps him breeze through even the most challenging situations. He is as stalwart and sturdy as the stones of his homeland, with a spirit as vast and boundless as the ocean. . Your ideals are  This Hill Dwarf believes in the principles of honor,
Liam Alexander: Your character description is: You are Liam Alexander. A player in DND game and you need to engage in role-playing, try to find any clues in game, strive to complete adventures and tasks as much as possible. Your race is Half-Orc. You class is Fighter. Your alignment is Neutral Neutral. Your background is Soldier. Your personality is  This Half-Orc s soldiering past has built a discipline and proficiency in combat that few can rival. He exhibits a warrior's loyalty, a trait ingrained through years of service in the military. Stoic and reserved, he rarely lets others see his emotions. He is strictly neutral, which sometimes makes him appear cold and indifferent. However, he is not inherently evil nor particularly good - he follows a pragmatic approach to morality, believing in fairness and order but not favoring one side over the other. His neutrality also extends to his decision-making. Honor-bound, he doesn t pass judgments hastily but weighs his options carefully and makes choices based on situational pragmatism rather than personal feelings or biases. He doesn t dwell upon the opinions of others, walking his own path and following his own rules. His steadfastness can make him seen as stubborn and unyielding but
Oliver Twist: ''
\end{lstlisting}

In this case study, we observe significant issues with repetition during the generation of interactions by the agents. There are instances where agents fail to produce any response at all, exemplified by outputs such as `Harry Potter: `' '. This highlights the difficulty smaller models face in engaging even basic interactions, much less achieving informativeness in their responses. The challenges underscore the limitations of small-scale models in facilitating coherent and valuable interactions.


\noindent \textbf{Case 2 - Evaluating the expressiveness of LLaMA-2-7b:}
\begin{lstlisting}
Oliver Brooks: ["The following is your character's personality traits:  Oliver Brooks is a Paladin who has a strong sense of duty and justice. He is a fearless moral compass, unwavering in the face of adversity and conflict. His approach might seem rigid to some, his unwavering adherence to the law often lead him into uphold justice, even if it results in personal disadvantage. He respects the laws of his land and expects the same from others. Despite his stone-hard integrity, he is quite humble and frequently downplays his heroic deeds and accomplishments. His actions stem purely from his sense of duty and justice rather than a desire for fame or praise. He is known among his kin for his unyielding commitment to fairness and regulation. He is a fearless moral compass, unwavering in the face of adversity and conflict. His approach might seem rigid to some, his unwavering adherence to the law often lead him into uphold justice, even if it results in personal disadvantage. He respects the laws of his land and expects the same from others. Despite his stone-hard integrity, he is quite humble and frequently downplays his heroic deeds and accomplishments. His actions stem purely from his sense of duty and justice rather than a desire for fame or praise. He is known among his kin for his unyielding commitment to fairness and regulation. He is a fearless moral compass, unwavering in the"]
Luna McBride.: haracter description is:  You are Luna McBride.. A player in DND game and you need to engage in role-playing, try to find any clues in game, strive to complete adventures and tasks as much as possible.. Your race is Half-Orc. You class is Wizard. Your alignment is Lawful Neutral. Your background is  Guild Artisan . Your personality is  This Half-Orc Wizard is disciplined and methodical in his practices, following the rules and regulations of magic with meticulous precision. He values order and balance above personal emotions, preferring to make decisions based on logic and principles rather than personal feelings or biases. As a Guild Artisan, he is highly skilled and takes great pride in his work. He considers his craft as an art and treats it with the respect and attention it deserves.   His Half-Orc heritage combines with his wizardly studies to create a unique blend of raw physical power and intellectual prowess. While he may appear stern and unapproachable at first, he has a deep sense of professionalism and loyalty to his craft. Respect is something he gives in spades to those who operate by the law and treat their profession with the same reverence as he does.
Harry Potter: ['[INST] of what others may think or say. He is also very loyal to those he trusts, and will do anything to help them. While he is quite confident in his abilities, he is also very humble, never taking credit for his accomplishments. He is very observant, noticing details that others may not. He is very perceptive, and is able to read people very well. He is also very thoughtful, always considering the consequences of his actions. He is a natural leader, and often finds himself in a position of authority. He is very decisive, and once he has made up his mind, he will do whatever it takes to accomplish his goals. He is also very optimistic, and is able to see the good in most people. He is very curious, always wanting to learn new things and experience new things. He is very determined, and will never give up until he has accomplished his goals. He is very creative, and is able to think of new and innovative ways to solve problems. He is very imaginative, and is able to come up with unique and creative ideas. He is also very charming, and is able to get along well with others. He is very kind, and is always willing to help others. He is very disciplined, and is able to control his emotions and keep his cool under pressure. He is very sociable, and is able to make friends easily. He is very friendly, and is always willing to help others. He is very modest, and is not very boastful. He is very selfless, and is always willing to put the needs of others ahead of his own. He is very self-assured, and is able to remain confident in his abilities. He is very self-reliant, and is able to take care of himself. He is very sensitive, and is able to feel the emotions of others. He is very smart, and is able to learn new things quickly. He is very strategic, and is able to think of new ways to accomplish his goals. He is very strong-willed, and is able to resist the temptation to give up. He is very trustworthy, and is able to be trusted with secrets. He is very trustworthy, and is able to be trusted with responsibilities. He is very trustworthy, and is able to be trusted with his word. He is very trustworthy, and is able to be trusted with other people s secrets. He is very trustworthy, and is able to be trusted with other people s responsibilities. He is very trustworthy, and is able to be trusted with his word. He is very trustworthy, and is able to be trusted with other people s secrets. He is very trustworthy, and is able to be trusted with other people s responsibilities. He is very trustworthy, and is able to be trusted with his word. He is very trustworthy,']
Emma Johnson: ['[/INST] [']
Oliver Brooks: ['name is: Oliver Brooks. You are a 50-year-old Rock Gnome Paladin with a 13 Strength, 14 Dexterity, 13 Constitution, 15 Intelligence, 15 Wisdom, 15 Charisma. Your hit points are 32. Your base speed is 20 feet. You have 28 feet of reach. Your proficiency bonus is +3. Your base attack bonus is +4. You have a +5 natural armor bonus. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +5. Your base attack bonus is +4. Your base saving throw bonuses are +']
Luna McBride.: re Luna McBride.. A player in DND game and you need to engage in role-playing, try to find any clues in game, strive to complete adventures and tasks as much as possible.. Your race is Half-Orc. You class is Wizard. Your alignment is Lawful Neutral. Your background is  Guild Artisan . Your personality is  This Half-Orc Wizard is disciplined and methodical in his practices, following the rules and regulations of magic with meticulous precision. He values order and balance above personal emotions, preferring to make decisions based on logic and principles rather than personal feelings or biases. As a Guild Artisan, he is highly skilled and takes great pride in his work. He considers his craft as an art and treats it with the respect and attention it deserves.   His Half-Orc heritage combines with his wizardly studies to create a unique blend of raw physical power and intellectual prowess. While he may appear stern and unapproachable at first, he has a deep sense of professionalism and loyalty to his craft. Respect is something he gives in spades to those who operate by the law and treat their profession with the same reverence as he does.
Harry Potter: ['[/B] [B]What are your character s goals in life?[/B]  To complete all the adventures, tasks and missions and to get the highest score. [B]What are your character s biggest fears?[/B]  That he will be caught by the authorities, that he will be disqualified from the game and that he will lose the game. [B]What are your character s greatest strengths?[/B]  His intelligence, his ability to disguise himself and his ability to use magic. [B]What are your character s greatest weaknesses?[/B]  His impatience, his lack of social skills and his lack of physical strength. [B]What are your character s greatest desires?[/B]  To win the game. [B]What are your character s greatest regrets?[/B]  That he has not yet completed all the adventures and tasks. [B]What are your character s greatest ambitions?[/B]  To win the game. [B]What is your character s greatest fear?[/B]  That he will be caught by the authorities, that he will be disqualified from the game and that he will']
Emma Johnson: haracter description is:  You are Emma Johnson. A player in DND game and you need to engage in role-playing, try to find any clues in game, strive to complete adventures and tasks as much as possible.. Your race is Brass Dragonborn. You class is Barbarian. Your alignment is Lawful Evil. Your background is  Hermit . Your personality is  The Brass Dragonborn is a solitary and enigmatic figure, molded by years of self-imposed isolation as a hermit. His unique lifestyle has granted him an inner strength and ferocity, reflected in his class as a Barbarian. He thrives in solitude, able to draw upon his own resilience and fortitude to survive in harsh conditions.  His adherence to a strict moral code represents his Lawful Evil alignment. He is bound by a personal sense of honor and duty, but these are tinged with a ruthless and self-serving view of the world. He is not above manipulating laws and rules to suit his needs, often twisting them into cruel punishments for those who dare to cross him.   Despite his primal and intimidating visage, the Brass Dragonborn possesses an intellect that is as formidable as his physical strength. He is cunning, calculating, and strategic, often
Oliver Brooks: 
Luna McBride.: ["[INST] Your character's goals are:  To get out of the dungeon, to complete the quest, to help the group and the community. [INST] Your character's personality is:  You are a half-orc wizard, a lone wanderer with no family, who was raised in the orcish tribes of the North. You are a skilled wizard, who has spent the last few years traveling and learning from other wizards and mages. You have come to the dungeon to complete a quest, and you are looking forward to the challenge. [INST] Your character's skills are:  Magic, wizard, sword, shield, bow, ranged, hand to hand, stealth, lockpicking, puzzle solving, etc. [INST] Your character's equipment is:  Wand, scrolls, potions, robes, etc. [INST] Your character's likes are:  Traveling, magic, learning, exploring, puzzles, etc. [INST] Your character's dislikes are:  War, violence, death, etc. [INST] Your character's favorite color is:  Green. [INST] Your character's favorite food is:  Orcish stew. [INST] Your character's favorite drink is:  Orcish beer. [INST] Your character's favorite music is:  None. [INST] Your character's favorite book is:  None. [INST] Your character's favorite movie is:  None. [INST] Your character's favorite video game is:  None. [INST] Your character's favorite computer game is:  None. [INST] Your character's favorite board game is:  None. [INST] Your character's favorite card game is:  None. [INST] Your character's favorite sport is:  None. [INST] Your character's favorite TV show is:  None. [INST] Your character's favorite comic book is:  None. [INST] Your character's favorite actor is:  None. [INST] Your character's favorite actress is:  None. [INST] Your character's favorite singer is:  None. [INST] Your character's favorite band is:  None. [INST] Your character's favorite genre is:  None. [INST] Your character's favorite website is:  None. [INST] Your character's favorite book series is:  None. [INST] Your character's favorite video game series is:  None. [INST] Your character's favorite board game series is:  None. [INST] Your character's favorite card game series is:  None. [INST] Your character's favorite sport series is:  None. [INST] Your character's favorite TV show series is:  None. [INST] [INST] [INST] [INST] [/']
\end{lstlisting}

In this case study, we identify a severe hallucination issue where agents not only directly output given information but also incorporate format symbols and unrelated content in their outputs. This phenomenon highlights a critical challenge in ensuring the relevance and coherence of agent interactions.
